Efficient Linearizability Checking for Actor-based Systems

Recent demand for distributed software had led to a surge in popularity in actor-based frameworks. However, even with the stylized message passing model of actors, writing correct distributed software is still difficult. We present our work on linearizability checking in DS2, an integrated framework for specifying, synthesizing, and testing distributed actor systems. The key insight of our approach is that often subcomponents of distributed actor systems represent common algorithms or data structures (e.g.\ a distributed hash table or tree) that can be validated against a simple sequential model of the system. This makes it easy for developers to validate their concurrent actor systems without complex specifications. DS2 automatically explores the concurrent schedules that system could arrive at, and it compares observed output of the system to ensure it is equivalent to what the sequential implementation could have produced. We describe DS2's linearizability checking and test it on several concurrent replication algorithms from the literature. We explore in detail how different algorithms for enumerating the model schedule space fare in finding bugs in actor systems, and we present our own refinements on algorithms for exploring actor system schedules that we show are effective in finding bugs.

==> Makefile <==
project=liviola

figs=

all: $(project).pdf

tex=$(wildcard *.tex)

PDFLATEXFLAGS	?= --interaction=nonstopmode --halt-on-error \
                   --file-line-error

$(project).pdf: $(tex) $(project).bbl
	pdflatex $(PDFLATEXFLAGS) $(project).tex
	pdflatex $(PDFLATEXFLAGS) $(project).tex
# mv sandstorm.pdf tmp.pdf
# gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite -sOutputFile=sandstorm.pdf tmp.pdf
# rm tmp.pdf

$(project).aux: $(tex) liviola.bib
	pdflatex $(PDFLATEXFLAGS) $(project).tex

$(project).bbl: liviola.bib $(project).aux
	-bibtex $(project)
	rm $(project).pdf

.PHONY: clean figs clean-figs

figs: $(figs)

figs-clean:
	-rm $(figs)

clean:
	-rm *.aux *.log *.bbl *.blg *.toc *.out $(project).pdf



==> figures/algorithms.fig.tex <==
\begin{figure}[b!]%[t!p]
  \centering
  \begin{minipage}[center]{1.0\linewidth}
    \centering
    \input{figures/ired.alg.fig}%
    \input{figures/transdpor.alg.fig}%
  \end{minipage}
\end{figure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> figures/algorithms_visualization.tex <==
\begin{figure}
  \centering
  \begin{subfigure}[b]{.48\textwidth}
    \centering \input{figures/history-picture2}
    \caption{H0, incomplete concurrent set history~\cite{linearizability:checker:go:porcupine}}
    \label{fig:histories:set:example:incomplete}
  \end{subfigure}  
  \begin{subfigure}[b]{.48\textwidth}
    \input{figures/wgl_picture.tex}
    \caption{WGL exploration of a linearizable history H1, 3 iterations}
    \label{fig:wgl1}
  \end{subfigure}
  \\
  \begin{subfigure}[b]{.9\textwidth}
    \input{figures/wgl_picture2.tex}
    \caption{WGL example exploration of a linearizable history H2, 6 iterations}
    \label{fig:wgl2}
  \end{subfigure}
  \\
  \begin{subfigure}[b]{.9\textwidth}
    \input{figures/wgl_picture3.tex}
    \caption{WGL exploration of a non-linearizable history H3, 15 iterations}
    \label{fig:wgl3}
  \end{subfigure}
  \caption{WGL algorithm examples}
  \label{fig:algorithm:example}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> figures/args-fig.tex <==
\begin{figure}[htb!]
\includegraphics[width=.45\textwidth]{figures/args-diagram.eps}
\caption{Fix as many variables using assumptions except for the subject.}
\label{fig:args}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> figures/calc_picture.tex <==
\begin{tikzpicture}
  % best length of a segment is 2.5cm
  \connect{1.55}{1.55}{1}{2.7}
  \invres{p(k1,1):ok}{1}{2.7}{1.5}{1}
  \connect{1.5}{0.75}{2.7}{3}
  \invres{g(k1):ok(1)}{3}{5}{0.75}{2}
  \invres{g(k1):ok(1)}{3.5}{5.5}{0}{3}
\end{tikzpicture}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> figures/calc_picture2.tex <==
\begin{tikzpicture}
  % best length of a segment is 2.5cm
  \connect{1.55}{1.55}{1}{2.7}
  \invres{p(k1,1):ok}{1}{2.7}{1.5}{1}
  \connect{1.5}{0.75}{2.7}{2.7}
  \invres{g(k1):ok(1)}{2.7}{5}{0.75}{2}
  \invres{g(k1):ok(1)}{3.0}{5.5}{0}{3}
  %
  \connect{1.55}{1.55}{6}{8}
  \invres{p(k1,2):ok}{6}{8}{1.5}{4}
  \connect{1.5}{.75}{8}{8.5}
  \connect{.8}{.8}{8.5}{11}
  \invres{g(k1):ok(2)}{8.5}{11}{0.75}{5}
  \connect{.75}{0}{11}{11.5}
  \connect{.05}{.05}{11.5}{13}
  \invres{g(k1):ok(2)}{11.5}{13}{0}{6}
\end{tikzpicture}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> figures/calc_picture3.tex <==
\begin{tikzpicture}
  % best length of a segment is 2.5cm
  \connect{1.55}{1.55}{1}{2.7}
  \invres{p(k1,1):ok}{1}{2.7}{1.5}{1}
  \connect{1.5}{0.75}{2.7}{2.7}
  \invres{g(k1):ok(1)}{2.7}{5}{0.75}{2}
  \invres{g(k1):ok(1)}{3.0}{5.5}{0}{3}
  %
  \connect{1.55}{1.55}{6}{8}
  \invres{p(k1,2):ok}{6}{8}{1.5}{4}
  \connect{1.5}{.75}{8}{8.5}
  \connect{.8}{.8}{8.5}{11}
  \invres{g(k1):ok(2)}{8.5}{11}{0.75}{5}
  \connect{.75}{0}{11}{11.5}
  \connect{.05}{.05}{11.5}{13}
  \invres{g(k1):ok(1)}{11.5}{13}{0}{6}
\end{tikzpicture}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> figures/histories-fig.tex <==
\begin{figure}[htb!]
  \subfloat[H1, a concurrent set
  history~\cite{linearizability:checker:go:porcupine}]{
    \label{fig:histories:set:example}
    \centering \input{figures/history-picture1}
  }
  \subfloat[H2, incomplete concurrent set
  history~\cite{linearizability:checker:go:porcupine}]{
    \label{fig:histories:set:example:incomplete}
    \centering \input{figures/history-picture2}
  }
  % \begin{subfigure}[b]{.48\textwidth}
  %   \centering \input{liviola/figures/history-picture1}
  %   \caption{H1, a concurrent set history~\cite{linearizability:checker:go:porcupine}}
  %   \label{fig:histories:set:example}
  % \end{subfigure}

  % \begin{subfigure}[b]{.48\textwidth}
  %   \centering \input{liviola/figures/history-picture2}
  %   \caption{H2, incomplete concurrent set history~\cite{linearizability:checker:go:porcupine}}
  %   \label{fig:histories:set:example:incomplete}
  % \end{subfigure}
  \caption{Multi-History example}
  \label{fig:histories}
\end{figure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> figures/history-picture1.tex <==
\begin{tikzpicture}
  % best length of a segment is 2.5cm
  \invres{set.insert(1):true}{1}{3.5}{1.5}{1}
  \invres{set.contains(1):true}{5}{8}{.75}{3}
  \invres{set.remove(1):false}{1.5}{4.5}{0}{2}
\end{tikzpicture}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> figures/history-picture2.tex <==
\begin{tikzpicture}
  % best length of a segment is 2.5cm
  \inv{add(1)}{1}{2}{1.5}{1}
  \invres{has(1):true}{3}{5}{.75}{3}
  \invres{rem(1):false}{1.5}{3.5}{0}{2}
\end{tikzpicture}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> figures/incomplete.histories.tex <==
\subfloat[\label{fig:incomplete:histories:histogram}]{ \centering \includegraphics[width=0.48\textwidth]{figures/incomplete.histories.eps} }

% \begin{subfigure}[b]{.48\textwidth}
%   \includegraphics{figures/incomplete.histories.eps}
%   \caption{\label{fig:incomplete:histories:histogram}}
% \end{subfigure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> figures/wgl_picture.tex <==
\begin{tikzpicture}
  % best length of a segment is 2.5cm
  \invres{p(k1,1):ok}{1}{2.7}{1.5}{1}
  % \connect{1.5}{0.75}{2.5}{2.7}
  \invres{g(k1):ok(1)}{3}{5}{0.75}{2}
  \invres{g(k1):ok(1)}{3.5}{5.5}{0}{3}
\end{tikzpicture}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> figures/wgl_picture2.tex <==
\begin{tikzpicture}
  % best length of a segment is 2.5cm
  \invres{p(k1,1):ok}{1}{2.7}{1.5}{1}
  \invres{g(k1):ok(1)}{2.7}{5}{0.75}{2}
  \invres{g(k1):ok(1)}{3.0}{5.5}{0}{3}
  %
  \invres{p(k1,2):ok}{6}{8}{1.5}{4}
  \invres{g(k1):ok(2)}{8.5}{11}{0.75}{5}
  \invres{g(k1):ok(2)}{11.5}{13}{0}{6}
\end{tikzpicture}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> figures/wgl_picture3.tex <==
\begin{tikzpicture}
  % best length of a segment is 2.5cm
  \invres{p(k1,1):ok}{1}{2.7}{1.5}{1}
  \invres{g(k1):ok(1)}{2.7}{5}{0.75}{2}
  \invres{g(k1):ok(1)}{3.0}{5.5}{0}{3}
  %
  \invres{p(k1,2):ok}{6}{8}{1.5}{4}
  \invres{g(k1):ok(2)}{8.5}{11}{0.75}{5}
  \invres{g(k1):ok(1)}{11.5}{13}{0}{6}
\end{tikzpicture}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> listings/pcomp-listing.tex <==
\begin{algorithm}
  \caption{WGL Linearizability Checker~\cite{linearizability:checker:go:porcupine,linearizability:checker:cpp,lowe:wgl:linearizability}}
  \begin{algorithmic}[1]
    \REQUIRE head\textunderscore entry.next points to history H first entry.
    \REQUIRE $N = 0.5 \times |H|$ is half the size of history H.
    \REQUIRE $linearized$ is a bitset such that $\forall k: 0 \leq k <
    N \Rightarrow linearized[k] = 0$
    \REQUIRE $\forall e \in H: 0 \leq id(e) < N$
    \REQUIRE $\forall e, e^\prime: id(e) = id(e^\prime)\Rightarrow e = e^\prime$
    \REQUIRE cache is an empty set
    \REQUIRE calls is an empty stack of entries
    \WHILE{head\textunderscore entry.next $\neq$ null}
    \IF{entry.match $\neq$ null}
    \STATE $\langle is\textunderscore linearizable, s^\prime \rangle = apply(entry,s)$
    \STATE $cache^\prime = copyOf(cache)$
    \IF{is\textunderscore linearizable}
    \STATE $linearized^\prime = copyOf(linearized)$
    \STATE $linearized^\prime[id(entry)] \leftarrow 1$
    \STATE $cache \leftarrow cache \cup \{\langle linearized^\prime, s^\prime\rangle\}$
    \ENDIF % end if(linearizable)
    \IF{$cache^\prime \neq cache$}
    \STATE $calls \leftarrow push(calls,\langle entry,s\rangle)$
    \STATE $s \leftarrow s^\prime$
    \STATE $linearized[id(entry)] \leftarrow 1$
    \STATE $LIFT(entry)$
    \STATE $entry \leftarrow head\textunderscore entry.next$
    \ELSE
    \STATE $entry \leftarrow head\textunderscore entry.next$
    \ENDIF % end second if
    \ELSE
    \IF{isEmpty(calls)}
    \RETURN false
    \ENDIF
    \STATE $\langle entry, s \rangle \leftarrow top(calls)$
    \STATE $linearized[id(entry)] \leftarrow 0$
    \STATE $calls \leftarrow pop(calls)$
    \STATE $UNLIFT(entry)$
    \STATE $entry \leftarrow entry.next$
    \ENDIF
    \ENDWHILE
    \RETURN true
  \end{algorithmic}
  \label{alg:wgl:pcomp}
\end{algorithm}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> summary.tex <==
\section{Summary}
In this section we provide a summary of the bold headlines marked by
this paper. The following are the main take away
points:
\begin{itemize}
\item \emph{Implementations of common distributed ADTs.}
  This work provides few real world implementations of common
  distributed ADTs in our executable model.
\item \emph{Stateful backtracking algorithms are feasible and we
    provided 7 of them in this work.} This is shown in experiments
  and the source code of the project~\cite{ds2:repo}.
\item \emph{Most bugs can reduce to race condition detection.} This is
  evident by the fact that even linearizability checking is a subset
  of data races of the globally shared state.
\item \emph{The model is effective and very efficient for large
    experiments.} As exemplified by all experiments and the 203 hrs
  running of one of IRed's harnesses without overly consuming too much
  memory above the normal level. Not to mention that all this paper's
  work also was done using only 4 rules, mentioned in the conclusion,
  out of the 16 formal operational semantics rules explained in
  a previous paper~\cite{ds2-opsem}.
\item \emph{The model is amenable to even deeper introspection.} As we
  could tell once limitations (\S\ref{sec:limitations}) are removed.
\item \emph{Extensible, modular, and composable algorithms.} Our
  schedulers are modularily implemented in order to enable composition
  of them cleanly to collaborate in an exploration, and to make them
  extensible to override their behaviors in minimal code writing, the
  code is in the DS2 repository~\cite{ds2:repo} and it speaks volumes without
  further ado.
\item \emph{Future enrichment.} We plan to populate even more
  algorithms and sample models in the code base to make it more
  feasible for the community to benefit and adopt it.
\item \emph{LiViola is not going to be last best.} We are confident
  that we as a community can do better than only LiViola and make
  similar or better improvements in other problems than linearizability
  checking. So we are looking forwards to seeing the framework grow.
\item \emph{Lessons learned.} Were presented and highlighted in the
  conclusion section..
\end{itemize}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "liviola"
%%% End:


==> tables/big-table-data.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> tables/big-table.tex <==
% ----------------------------------------
% Below is the table with SR intact
% ----------------------------------------

\begin{table}[h!]
  \centering
  \tiny
  \begin{tabular}{| l | c || c  c  c  c  c  c  c | c  c c   c  c  c c ||} \cline{2-16}
    \multicolumn{1}{l|}{}& \textbf{\#Inv.}
    & \multicolumn{7}{c |}{\textbf{2R+1W}}
    & \multicolumn{7}{c |}{\textbf{2R+2W}}\\ \cline{2-16}
    \multicolumn{1}{l|}{}& \textbf{Alg.}
    & \textbf{EX} & \textbf{SR} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV}
    & \textbf{EX} & \textbf{SR} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV} \\ \hline
    \multirow{13}{1cm}{\textbf{Dist. Reg.}
      % \newline \#S = 10K
    \newline \#Agents = 2
    \newline \#Rtry = 3
    \newline Qrm = 2 }            %                  EX1     SR1       DB1     DP1        TD1      IR1       LV1     EX2      SR2     DB2     DP2     TD2     IR2      LV2
                                  & \textbf{\#S}  & 4,200  & 100K   & 4,200  & 2,984   & 2,906   & 2,906   & 88    & 50K    & 100K  & 50K   &  50K & 50K   &  50K  & 7,236 \\ \cline{2-16}
                                  & \textbf{\#IH} & 4,195  &  0     & 4,195  & 2,979   & 2,901   & 2,901   & 83    & 50K    & 100K  & 50K   & 50K  & 50K   &  50K  & 7,236 \\ \cline{2-16}
                                  & \textbf{\#UH} &   37   &  26    &   37   &   37    &   37    &   37    & 22    & 8      &   91  &  8    &  8   &  8    &  8    &  147  \\ \cline{2-16}
                                  & \textbf{\#NL} &   0    &  0     &   0    &   0     &   0     &   0     &  0    & 0      &  0    &  0    &  0   &  0    &  0    &  0    \\ \cline{2-16}
                                  & \textbf{NL/UH}&  0.0 \%&  0.0\% &   0.0\%&    0.0\%&  0.0\%  &   0.0\% & 0.0\% &  0.0\% & 0.0\% & 0.0\% & 0.0\%& 0.0\% & 0.0\% & 0.0\% \\ \cline{2-16}
                                  & \textbf{UH/S} &  0.88\%&  0.03\%&  0.88\%&  1.24\% &  1.27\% &  1.27\% & 25.0\%& 0.02\% & 0.09\%& 0.02\%&0.02\%& 0.02\%& 0.02\%& 2.03\%\\ \cline{2-16}
                                  & \textbf{NL/S} & 0.0\%  &  0.0\% & 0.0\%  &   0.0\% &  0.0\%  &  0.0\%  & 0.0\% &  0.0\% & 0.0\% & 0.0\% &0.0\% & 0.0\% & 0.0\% & 0.0\% \\ \cline{2-16}
                                  & \textbf{TS}   & 0:06   & 4:48   & 0:06   & 0:05    & 0:05    & 0:04    & 0:00  & 1:27   & 5:49  & 1:22  & 1:36 & 1:34  & 1:34  & 0:09  \\ \cline{2-16}
                                  & \textbf{ST}   & 0:18   & 1:52   & 0:21   & 0:12    & 0:13    & 0:17    & 0:00  & 9:27   & 2:55  & 6:27  & 7:09 & 7:42  & 7:05  & 0:34  \\ \cline{2-16}
                                  & \textbf{TC}   & 0:00   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00  & 0:00   & 0:00  & 0:00  & 0:00 & 0:00  & 0:00  & 0:00  \\ \cline{2-16}
                                  & \textbf{TT}   & 0:06   & 4:48   & 0:06   & 0:05    & 0:05    & 0:04    & 0:00  & 1:27   & 5:49  & 1:22  & 1:36 & 1:34  & 1:34  & 0:09  \\ \cline{2-16}
                                  & \textbf{\#HF} &  -     &  -     & -      & -       &  -      &   -     &  -    & -      &  -    &  -    &  -   &  -    &  -    &  -    \\ \cline{2-16}
                                  & \textbf{TF}   & 0:00   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00  & 0:00   & 0:00  & 0:00  & 0:00 & 0:00  & 0:00  & 0:00  \\ \cline{2-16} \hline
% ========================================================================================================================
    \multicolumn{1}{l|}{}& \textbf{Alg.}
    & \textbf{EX} & \textbf{SR} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV}
    & \textbf{EX} & \textbf{SR} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV} \\ \hline
    \multirow{13}{1cm}{\textbf{Err. Dist. Reg.}
      % \newline \#S = 10K
    \newline \#Agents = 3
    \newline \#Rtry = 3
    \newline Qrm = 2 \\fixed Qrm\\regardless \\of agents \\count }
                                                    % EX1     SR1       DB1     DP1        TD1      IR1       LV1     EX2      SR2     DB2     DP2     TD2     IR2      LV2
                                  & \textbf{\#S}  &  252   &  100K  &  252   &  20     &   20    &  14     &  14    &  50K   &  100K &  50K  & 50K   &  50K  &30,063 & 28,517\\ \cline{2-16}
                                  & \textbf{\#IH} &  247   &   0    &  247   &  15     &   15    &  11     &  11    & 49,996 &   0   & 49,996&49,894 & 49,875&29,995 & 28,441\\ \cline{2-16}
                                  & \textbf{\#UH} &  11    &   66   &  11    &  11     &   12    &  8      &  8     &  20    &  459  &  18   &  79   &  152  &  97   &  116  \\ \cline{2-16}
                                  & \textbf{\#NL} &   2    &   0    &   2    &   3     &   4     &  2      &  2     &  0     &  0    &  0    &  11   &  18   & 6     &  10   \\ \cline{2-16}
                                  & \textbf{NL/UH}& 18.18\%&  0.0\% & 18.18\%&  27.27\%& 33.33\% &  25.0\% & 25.0\% &  0.0\% & 0.0\% & 0.0\% &13.92\%&11.84\%& 6.19\%& 8.62\%\\ \cline{2-16}
                                  & \textbf{UH/S} & 4.37\% &  0.07\%& 4.37\% &  55.0\% & 60.0\%  &  57.14\%&57.14\% & 0.04\% & 0.46\%& 0.04\%& 0.16\%& 0.3\% & 0.32\%& 0.41\%\\ \cline{2-16}
                                  & \textbf{NL/S} & 0.79\% &  0.0\% & 0.79\% &  15.0\% & 20.0\%  &  14.29\%&14.29\% & 0.0\%  & 0.0\% & 0.0\% & 0.02\%& 0.04\%& 0.02\%& 0.04\%\\ \cline{2-16}
                                  & \textbf{TS}   & 0:00   & 4:09   & 0:00   & 0:00    & 0:00    & 0:00    &  0:00  & 1:31   & 4:34  & 1:50  & 1:48  & 1:46  & 1:11  & 1:13  \\ \cline{2-16}
                                  & \textbf{ST}   & 0:01   & 1:39   & 0:01   & 0:00    & 0:00    & 0:00    &  0:00  & 5:19   & 2:00  & 5:56  & 6:29  & 5:46  & 3:01  & 3:02  \\ \cline{2-16}
                                  & \textbf{TC}   & 0:00   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    &  0:00  & 0:00   & 0:00  & 0:00  & 0:00  & 0:00  & 0:00  & 0:00  \\ \cline{2-16}
                                  & \textbf{TT}   & 0:00   & 4:09   & 0:00   & 0:00    & 0:00    & 0:00    &  0:00  & o1:31  & 4:34  & 1:50  & 1:48  & 1:46  & 1:11  & 1:13  \\ \cline{2-16}
                                  & \textbf{\#HF} &  2     &  -     &  2     &   0     &  0      &   1     &  1     &  -     &  -    &   -   &  0    &  0    &  0    &  0    \\ \cline{2-16}
                                  & \textbf{TF}   & 0:00   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00   & 0:00   & 0:00  & 0:00  & 0:00  & 0:00  & 0:00  & 0:00  \\ \cline{2-16} \hline
% ========================================================================================================================
    % \cline{2-16}
    \multicolumn{1}{l|}{}& \textbf{Alg.}
    & \textbf{EX} & \textbf{SR} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV}
    & \textbf{EX} & \textbf{SR} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV} \\ \hline
    \multirow{13}{1cm}{\textbf{Another Dist. Reg.}
      % \newline \#S = 10K
    \newline \#Agents = 2
    \newline \#Rtry = 3
    \newline Qrm = 2 }            %                  EX1     SR1       DB1     DP1        TD1      IR1       LV1     EX2      SR2     DB2     DP2     TD2     IR2      LV2
                                  & \textbf{\#S}  & 1,680  & 100K   & 1,680  & 908     &  818    &  802    & 802    &  50K   &  100K &  50K  &  50K   & 50K   &  50K  & 50K   \\ \cline{2-16}
                                  & \textbf{\#IH} & 887    &  0     &   887  & 462     &  419    &  412    & 412    & 42,890 & 95,060& 42,890& 40,152 & 39,564& 39,884& 39,884\\ \cline{2-16}
                                  & \textbf{\#UH} & 148    &  28    &   148  & 140     &  132    &   124   & 124    &   718  &  131  &  718  &  1,610 & 1,876 & 1,907 & 1,907 \\ \cline{2-16}
                                  & \textbf{\#NL} &  0     &  0     &   0    &   0     &   0     &   0     &  0     &    0   &  0    &  0    &  0     & 0     &  0    & 0     \\ \cline{2-16}
                                  & \textbf{NL/UH}& 0.0\%  &  0.0\% &  0.0\% &  0.0\%  &  0.0\%  &  0.0\%  & 0.0\%  &  0.0\% & 0.0\% & 0.0\% &0.0\%   & 0.0\% & 0.0\% & 0.0\% \\ \cline{2-16}
                                  & \textbf{UH/S} & 8.81\% &  0.03\%& 8.81\% & 15.42\% & 16.14\% & 15.46\% &15.46\% & 1.44\% & 0.13\%& 1.44\%&3.22\%  & 3.75\%& 3.81\%& 3.81\%\\ \cline{2-16}
                                  & \textbf{NL/S} & 0.0\%  &  0.0\% & 0.0\%  &  0.0\%  &   0.0\% &  0.0\%  & 0.0\%  &  0.0\% & 0.0\% & 0.0\% &0.0\%   & 0.0\% & 0.0\% & 0.0\% \\ \cline{2-16}
                                  & \textbf{TS}   & 0:22   & 8:54   & 0:20   & 0:06    & 0:07    & 0:07    & 0:07   & 693:56 & 4:44  & 660:41&876:36  & 835:39& 859:53& 845:30\\ \cline{2-16}
                                  & \textbf{ST}   & 1:12   & 1:10   & 1:07   & 0:19    & 0:21    & 0:20    & 0:22   &2635:48 & 1:52  &2608:10&2871:33 &2703:56&2889:04&2857:07\\ \cline{2-16}
                                  & \textbf{TC}   & 0:00   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00   & 0:00   & 0:00  & 0:00  & 0:00   & 0:00  & 0:00  & 0:00  \\ \cline{2-16}
                                  & \textbf{TT}   & 0:22   & 8:54   & 0:20   & 0:06    & 0:07    & 0:07    & 0:07   & 693:56 & 4:44  & 660:41& 876:36 & 835:39& 859:53& 845:30\\ \cline{2-16}
                                  & \textbf{\#HF} &   -    &  -     & -      & -       & -       & -       & -      &  -     & -     & -     &  -     &  -    &  -    &  -    \\ \cline{2-16}
                                  & \textbf{TF}   & 0:00   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00   & 0:00   & 0:00  & 0:00  & 0:00   & 0:00  & 0:00  & 0:00  \\ \cline{2-16} \hline
% ========================================================================================================================
    \multicolumn{1}{l|}{}& \textbf{Alg.}
    & \textbf{EX} & \textbf{SR} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV}
    & \textbf{EX} & \textbf{SR} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV} \\ \hline
    \multirow{13}{1cm}{\textbf{Paxos}
      % \newline \#S = 10K
    \newline \#Agents = 2
    \newline \#Rtry = *
    \newline Qrm = majority }     %                  EX1     SR1       DB1     DP1        TD1      IR1       LV1     EX2      SR2     DB2     DP2     TD2     IR2      LV2
                                  & \textbf{\#S}  &  50K   & 100K   &  50K   &  50K    & 50K     &   50K   &  50K  & 50K    &  100K & 50K   & 50K  &  50K  &  50K  &  50K  \\ \cline{2-16}
                                  & \textbf{\#IH} &  0     &  0     &  0     &   0     &  0      &   0     &  0    &  0     &   0   &  0    &  0   &  0    &   0   &   0   \\ \cline{2-16}
                                  & \textbf{\#UH} &  14    &  26    &   14   &  12     &  12     &   12    &  12   &  6     &  85   &  6    &  6   &  6    &   6   &   9   \\ \cline{2-16}
                                  & \textbf{\#NL} &   0    &  0     &   0    &   0     &   0     &   0     &   0   &  0     &  0    &  0    &  0   &  0    &   0   &   0   \\ \cline{2-16}
                                  & \textbf{NL/UH}&  0.0\% &  0.0\% &  0.0\% &   0.0\% &   0.0\% &   0.0\% & 0.0\% & 0.0\%  & 0.0\% & 0.0\% &0.0\% & 0.0\% & 0.0\% & 0.0\% \\ \cline{2-16}
                                  & \textbf{UH/S} & 0.03\% &  0.03\%&  0.03\%&  0.02\% &   0.02\%&   0.02\%& 0.02\%& 0.01\% & 0.08\%& 0.01\%&0.01\%& 0.01\%& 0.01\%& 0.02\%\\ \cline{2-16}
                                  & \textbf{NL/S} & 0.0\%  &  0.0\% &  0.0\% &  0.0\%  &   0.0\% &   0.0\% & 0,0\% & 0.0\%  & 0.0\% & 0.0\% &0.0\% & 0.0\% & 0.0\% & 0.0\% \\ \cline{2-16}
                                  & \textbf{TS}   & 68:19  & 6:25   & 67:51  & 74:44   & 32:15   & 80:51   & 76:13 & 35:54  & 6:12  & 35:28 & 56:50& 57:22 &70:57  & 75:48 \\ \cline{2-16}
                                  & \textbf{ST}   & 306:30 & 3:22   & 318:48 & 332:29  & 149:52  &350:19   & 325:29& 286:39 & 3:40  & 307:22&581:43& 570:32&706:18 & 635:05\\ \cline{2-16}
                                  & \textbf{TC}   & 0:00   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00  & 0:00   & 0:00  & 0:00  & 0:00 & 0:00  & 0:00  & 0:00  \\ \cline{2-16}
                                  & \textbf{TT}   & 68:19  & 6:25   & 67:51  & 74:44   & 32:15   &80:51    & 76:13 & 35:54  & 6:12  & 35:28 &56:50 & 57:22 & 70:57 & 75:48 \\ \cline{2-16}
                                  & \textbf{\#HF} &   -    &  -     & -      & -       & -       &   -     &  -    &   -    &   -   &   -   &  -   &   -   &   -   &   -   \\ \cline{2-16}
                                  & \textbf{TF}   & 0:00   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00  & 0:00   & 0:00  & 0:00  & 0:00 & 0:00  & 0:00  & 0:00  \\ \cline{2-16} \hline 
% ========================================================================================================================
    \multicolumn{1}{l|}{}& \textbf{Alg.}
    & \textbf{EX} & \textbf{SR} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV}
    & \textbf{EX} & \textbf{SR} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV} \\ \hline
    \multirow{13}{1cm}{\textbf{Open Chord}
      % \newline \#S = 10K
    \newline \#Agents = 2
    \newline \#Rtry = N/A
    \newline Qrm = N/A}           %                  EX1     SR1       DB1     DP1        TD1      IR1       LV1     EX2      SR2     DB2     DP2     TD2     IR2      LV2
                                  & \textbf{\#S}  & 18,396 &  100K  & 18,396 &  5,926  & 2,633   &  1,935  & 21    & 50K    &  100K &  50K  &  50K   &  50K  & 50K   & 71    \\ \cline{2-16}
                                  & \textbf{\#IH} &   0    &  0     &   0    &   0     & 0       &  0      &  0    & 0      &   0   & 0     & 0      &  0    &  0    &  0    \\ \cline{2-16}
                                  & \textbf{\#UH} &  165   & 35     &  165   &   143   &  117    &  121    & 17    & 325    & 329   & 3557  & 1073   &  1034 & 1498  &  49   \\ \cline{2-16}
                                  & \textbf{\#NL} &  17    &  0     &  17    &   16    &  14     &  12     &  4    &  15    &  1    &  357  &  181   &  163  & 295   &  1    \\ \cline{2-16}
                                  & \textbf{NL/UH}&  10.3\%&  0.0\% & 10.3\% & 11.19\% & 11.97\% &  9.92\% &23.53\%& 4.62\% & 0.3\% &10.04\%&16.87\% &15.76\%&19.69\%& 2.04\%\\ \cline{2-16}
                                  & \textbf{UH/S} &  0.9\% & 0.03\% & 0.9\%  &  2.41\% & 4.44\%  &  6.25\% &80.95\%& 0.65\% & 0.33\%& 7.11\%& 2.15\% &2.07\% & 3.0\% &69.01\%\\ \cline{2-16}
                                  & \textbf{NL/S} & 0.09\% &  0.0\% & 0.09\% &  0.27\% & 0.53\%  &  0.62\% &19.05\%& 0.03\% & 0.0\% & 0.71\%& 0.36\% & 0.33\%& 0.59\%& 1.41\%\\ \cline{2-16}
                                  & \textbf{TS}   & 5:30   & 6:30   & 5:34   & 0:43    & 0:10    & 0:06    & 0:00  & 73:29  & 7:40  & 34:01 & 50:48  & 60:03 & 100:43& 0:00  \\ \cline{2-16}
                                  & \textbf{ST}   & 18:25  & 3:40   & 17:56  & 2:04    & 0:34    & 0:24    & 0:00  & 323:39 & 4:43  & 138:25& 194:59 & 214:55& 359:59& 0:00  \\ \cline{2-16}
                                  & \textbf{TC}   & 0:00   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00  & 0:00   & 0:00  & 0:00  & 0:00   & 0:00  & 0:00  & 0:00  \\ \cline{2-16}
                                  & \textbf{TT}   & 5:30   & 6:30   & 5:34   & 0:43    & 0:10    & 0:06    & 0:00  & 73:29  & 7:40  & 34:02 & 50:48  & 60:03 & 100:43& 0:00  \\ \cline{2-16}
                                  & \textbf{\#HF} &   15   &   -    &   15   &  12     &    10   &  12     &   0   & 15     & 168   &   1   &  2     &  9    &   1   &   22  \\ \cline{2-16}
                                  & \textbf{TF}   & 0:00   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00  & 0:00   & 0:00  & 0:00  & 0:00   & 0:00  & 0:00  & 0:00  \\ \cline{2-16} \hline
% ========================================================================================================================
    \multicolumn{1}{l|}{}& \textbf{Alg.}
    & \textbf{EX} & \textbf{SR} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV}
    & \textbf{EX} & \textbf{SR} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV} \\ \cline{2-16}

  \end{tabular}
  \caption{\scriptsize
    This table shows 7 schedulers bench marked against 5
distributed systems. The following is the legend for the symbols in the table:
\textbf{Schedulers:} (EX) Exhaustive, (SR) Systematic Random, (DB)
Delay-Bounded, (DP) DPOR, (TD) TransDPOR, (IR) IRed , (LV)
LiViola. \textbf{Per Benchmark symbols/numbers:} (\#Inv.) No. of
Invocations, (R-W) the comparison of reads requests compared to write
requests, (\#S) No. of Schedules, (\#UH) No. of Unique Histories,
(\#NL) No. of Non-Linearizable histories, (NL/UH) None-Linearizable to
Unique Histories, (\#IH) No. of Incomplete histories, (NL/S) ration of
Non-Linearizable histories to No. of Schedules, (UH/S) Ration of
No. of Unique Histories to No. of Schedules generated, (\#Rtry) No. of
Retries, (Qrm) number of agents forming the Quorum if applicable, (TS)
Time to generate all Schedules (mm:ss), (ST) time to produce same
schedules by an otherwise a stateless variant of the algorithm, (TC)
Time to check all unique histories (mm:ss), (TT) Total Time = TS + TC
(mm:ss),(\#HF) No. of histories until first buggy history,(TF) time to
find the First buggy history by WGL algorithm (mm:ss), that is the sum
of time needed to check all histories before and including the first
buggy one. Note that the number of agents in all these benchmarks was
limited to 5. The subcolumns headers e.g. 2r+1w stands for 2 reads and
1 write test harness.
  } % end caption
  \label{big:table:benchmarks}
\end{table}

% ----------------------------------------
% Below is the table with out SR intact
% ----------------------------------------


% \begin{table}[htb!]
%   \centering
%   \tiny
%   \begin{tabular}{| l | c || c  c  c  c  c  c | c  c  c  c  c c ||} \cline{2-14}
%     \multicolumn{1}{l|}{}& \textbf{\#Inv.}
%     & \multicolumn{6}{c |}{\textbf{2R+1W}}
%     & \multicolumn{6}{c |}{\textbf{2R+2W}}\\ \cline{2-14}
%     \multicolumn{1}{l|}{}& \textbf{Alg.}
%     & \textbf{EX} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV}
%     & \textbf{EX} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV} \\ \hline
%     \multirow{13}{1cm}{\textbf{Dist. Reg.}
%       % \newline \#S = 10K
%     \newline \#Agents = 2
%     \newline \#Rtry = 3
%     \newline Qrm = 2 }            %                  EX1      DB1     DP1        TD1      IR1       LV1     EX2      DB2     DP2     TD2     IR2      LV2
%                                   & \textbf{\#S}  & 4,200  & 4,200  & 2,984   & 2,906   & 2,906   & 88    & 50K    & 50K   &  50K & 50K   &  50K  & 7,236 \\ \cline{2-14}
%                                   & \textbf{\#IH} & 4,195  & 4,195  & 2,979   & 2,901   & 2,901   & 83    & 50K    & 50K   & 50K  & 50K   &  50K  & 7,236 \\ \cline{2-14}
%                                   & \textbf{\#UH} &   37   &   37   &   37    &   37    &   37    & 22    & 8      &  8    &  8   &  8    &  8    &  147  \\ \cline{2-14}
%                                   & \textbf{\#NL} &   0    &   0    &   0     &   0     &   0     &  0    & 0      &  0    &  0   &  0    &  0    &  0    \\ \cline{2-14}
%                                   & \textbf{NL/UH}&  0.0 \%&   0.0\%&    0.0\%&  0.0\%  &   0.0\% & 0.0\% &  0.0\% & 0.0\% & 0.0\%& 0.0\% & 0.0\% & 0.0\% \\ \cline{2-14}
%                                   & \textbf{UH/S} &  0.88\%&  0.88\%&  1.24\% &  1.27\% &  1.27\% & 25.0\%& 0.02\% & 0.02\%&0.02\%& 0.02\%& 0.02\%& 2.03\%\\ \cline{2-14}
%                                   & \textbf{NL/S} & 0.0\%  & 0.0\%  &   0.0\% &  0.0\%  &  0.0\%  & 0.0\% &  0.0\% & 0.0\% &0.0\% & 0.0\% & 0.0\% & 0.0\% \\ \cline{2-14}
%                                   & \textbf{TS}   & 0:06   & 0:06   & 0:05    & 0:05    & 0:04    & 0:00  & 1:27   & 1:22  & 1:36 & 1:34  & 1:34  & 0:09  \\ \cline{2-14}
%                                   & \textbf{ST}   & 0:18   & 0:21   & 0:12    & 0:13    & 0:17    & 0:00  & 9:27   & 6:27  & 7:09 & 7:42  & 7:05  & 0:34  \\ \cline{2-14}
%                                   & \textbf{TC}   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00  & 0:00   & 0:00  & 0:00 & 0:00  & 0:00  & 0:00  \\ \cline{2-14}
%                                   & \textbf{TT}   & 0:06   & 0:06   & 0:05    & 0:05    & 0:04    & 0:00  & 1:27   & 1:22  & 1:36 & 1:34  & 1:34  & 0:09  \\ \cline{2-14}
%                                   & \textbf{\#HF} &  -     & -      & -       &  -      &   -     &  -    & -      &  -    &  -   &  -    &  -    &  -    \\ \cline{2-14}
%                                   & \textbf{TF}   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00  & 0:00   & 0:00  & 0:00 & 0:00  & 0:00  & 0:00  \\ \cline{2-14} \hline
% % ========================================================================================================================
%     \multicolumn{1}{l|}{}& \textbf{Alg.}
%     & \textbf{EX} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV}
%     & \textbf{EX} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV} \\ \hline
%     \multirow{13}{1cm}{\textbf{Err. Dist. Reg.}
%       % \newline \#S = 10K
%     \newline \#Agents = 3
%     \newline \#Rtry = 3
%     \newline Qrm = 2 \\fixed}
%                                                     % EX1     DB1     DP1        TD1      IR1       LV1     EX2        DB2     DP2     TD2     IR2      LV2
%                                   & \textbf{\#S}  &  252   &  252   &  20     &   20    &  14     &  14    &  50K   &  50K  & 50K   &  50K  &30,063 & 28,517\\ \cline{2-14}
%                                   & \textbf{\#IH} &  247   &  247   &  15     &   15    &  11     &  11    & 49,996 & 49,996&49,894 & 49,875&29,995 & 28,441\\ \cline{2-14}
%                                   & \textbf{\#UH} &  11    &  11    &  11     &   12    &  8      &  8     &  20    &  18   &  79   &  152  &  97   &  116  \\ \cline{2-14}
%                                   & \textbf{\#NL} &   2    &   2    &   3     &   4     &  2      &  2     &  0     &  0    &  11   &  18   & 6     &  10   \\ \cline{2-14}
%                                   & \textbf{NL/UH}& 18.18\%& 18.18\%&  27.27\%& 33.33\% &  25.0\% & 25.0\% &  0.0\% & 0.0\% &13.92\%&11.84\%& 6.19\%& 8.62\%\\ \cline{2-14}
%                                   & \textbf{UH/S} & 4.37\% & 4.37\% &  55.0\% & 60.0\%  &  57.14\%&57.14\% & 0.04\% & 0.04\%& 0.16\%& 0.3\% & 0.32\%& 0.41\%\\ \cline{2-14}
%                                   & \textbf{NL/S} & 0.79\% & 0.79\% &  15.0\% & 20.0\%  &  14.29\%&14.29\% & 0.0\%  & 0.0\% & 0.02\%& 0.04\%& 0.02\%& 0.04\%\\ \cline{2-14}
%                                   & \textbf{TS}   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    &  0:00  & 1:31   & 1:50  & 1:48  & 1:46  & 1:11  & 1:13  \\ \cline{2-14}
%                                   & \textbf{ST}   & 0:01   & 0:01   & 0:00    & 0:00    & 0:00    &  0:00  & 5:19   & 5:56  & 6:29  & 5:46  & 3:01  & 3:02  \\ \cline{2-14}
%                                   & \textbf{TC}   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    &  0:00  & 0:00   & 0:00  & 0:00  & 0:00  & 0:00  & 0:00  \\ \cline{2-14}
%                                   & \textbf{TT}   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    &  0:00  & o1:31  & 1:50  & 1:48  & 1:46  & 1:11  & 1:13  \\ \cline{2-14}
%                                   & \textbf{\#HF} &  2     &  2     &   0     &  0      &   1     &  1     &  -     &   -   &  0    &  0    &  0    &  0    \\ \cline{2-14}
%                                   & \textbf{TF}   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00   & 0:00   & 0:00  & 0:00  & 0:00  & 0:00  & 0:00  \\ \cline{2-14} \hline
% % ========================================================================================================================
%     % \cline{2-16}
%     \multicolumn{1}{l|}{}& \textbf{Alg.}
%     & \textbf{EX} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV}
%     & \textbf{EX} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV} \\ \hline
%     \multirow{13}{1cm}{\textbf{Another Dist. Reg.}
%       % \newline \#S = 10K
%     \newline \#Agents = 2
%     \newline \#Rtry = 3
%     \newline Qrm = 2 }            %                  EX1       DB1     DP1        TD1      IR1       LV1     EX2       DB2     DP2     TD2     IR2      LV2
%                                   & \textbf{\#S}  & 1,680  & 1,680  & 908     &  818    &  802    & 802    &  50K   &  50K  &  50K   & 50K   &  50K  & 50K   \\ \cline{2-14}
%                                   & \textbf{\#IH} & 887    &   887  & 462     &  419    &  412    & 412    & 42,890 & 42,890& 40,152 & 39,564& 39,884& 39,884\\ \cline{2-14}
%                                   & \textbf{\#UH} & 148    &   148  & 140     &  132    &   124   & 124    &   718  &  718  &  1,610 & 1,876 & 1,907 & 1,907 \\ \cline{2-14}
%                                   & \textbf{\#NL} &  0     &   0    &   0     &   0     &   0     &  0     &    0   &  0    &  0     & 0     &  0    & 0     \\ \cline{2-14}
%                                   & \textbf{NL/UH}& 0.0\%  &  0.0\% &  0.0\%  &  0.0\%  &  0.0\%  & 0.0\%  &  0.0\% & 0.0\% &0.0\%   & 0.0\% & 0.0\% & 0.0\% \\ \cline{2-14}
%                                   & \textbf{UH/S} & 8.81\% & 8.81\% & 15.42\% & 16.14\% & 15.46\% &15.46\% & 1.44\% & 1.44\%&3.22\%  & 3.75\%& 3.81\%& 3.81\%\\ \cline{2-14}
%                                   & \textbf{NL/S} & 0.0\%  & 0.0\%  &  0.0\%  &   0.0\% &  0.0\%  & 0.0\%  &  0.0\% & 0.0\% &0.0\%   & 0.0\% & 0.0\% & 0.0\% \\ \cline{2-14}
%                                   & \textbf{TS}   & 0:22   & 0:20   & 0:06    & 0:07    & 0:07    & 0:07   & 693:56 & 660:41&876:36  & 835:39& 859:53& 845:30\\ \cline{2-14}
%                                   & \textbf{ST}   & 1:12   & 1:07   & 0:19    & 0:21    & 0:20    & 0:22   &2635:48 &2608:10&2871:33 &2703:56&2889:04&2857:07\\ \cline{2-14}
%                                   & \textbf{TC}   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00   & 0:00   & 0:00  & 0:00   & 0:00  & 0:00  & 0:00  \\ \cline{2-14}
%                                   & \textbf{TT}   & 0:22   & 0:20   & 0:06    & 0:07    & 0:07    & 0:07   & 693:56 & 660:41& 876:36 & 835:39& 859:53& 845:30\\ \cline{2-14}
%                                   & \textbf{\#HF} &   -    & -      & -       & -       & -       & -      &  -     & -     &  -     &  -    &  -    &  -    \\ \cline{2-14}
%                                   & \textbf{TF}   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00   & 0:00   & 0:00  & 0:00   & 0:00  & 0:00  & 0:00  \\ \cline{2-14} \hline
% % ========================================================================================================================
%     \multicolumn{1}{l|}{}& \textbf{Alg.}
%     & \textbf{EX} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV}
%     & \textbf{EX} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV} \\ \hline
%     \multirow{13}{1cm}{\textbf{Paxos}
%       % \newline \#S = 10K
%     \newline \#Agents = 2
%     \newline \#Rtry = *
%     \newline Qrm = majority }     %                  EX1       DB1     DP1        TD1      IR1       LV1     EX2      DB2     DP2     TD2     IR2    LV2
%                                   & \textbf{\#S}  &  50K   &  50K   &  50K    & 50K     &   50K   &  50K  & 50K    & 50K   & 50K  &  50K  &  50K  &  50K  \\ \cline{2-14}
%                                   & \textbf{\#IH} &  0     &  0     &   0     &  0      &   0     &  0    &  0     &  0    &  0   &  0    &   0   &   0   \\ \cline{2-14}
%                                   & \textbf{\#UH} &  14    &   14   &  12     &  12     &   12    &  12   &  6     &  6    &  6   &  6    &   6   &   9   \\ \cline{2-14}
%                                   & \textbf{\#NL} &   0    &   0    &   0     &   0     &   0     &   0   &  0     &  0    &  0   &  0    &   0   &   0   \\ \cline{2-14}
%                                   & \textbf{NL/UH}&  0.0\% &  0.0\% &   0.0\% &   0.0\% &   0.0\% & 0.0\% & 0.0\%  & 0.0\% &0.0\% & 0.0\% & 0.0\% & 0.0\% \\ \cline{2-14}
%                                   & \textbf{UH/S} & 0.03\% &  0.03\%&  0.02\% &   0.02\%&   0.02\%& 0.02\%& 0.01\% & 0.01\%&0.01\%& 0.01\%& 0.01\%& 0.02\%\\ \cline{2-14}
%                                   & \textbf{NL/S} & 0.0\%  &  0.0\% &  0.0\%  &   0.0\% &   0.0\% & 0,0\% & 0.0\%  & 0.0\% &0.0\% & 0.0\% & 0.0\% & 0.0\% \\ \cline{2-14}
%                                   & \textbf{TS}   & 68:19  & 67:51  & 74:44   & 32:15   & 80:51   & 76:13 & 35:54  & 35:28 & 56:50& 57:22 &70:57  & 75:48 \\ \cline{2-14}
%                                   & \textbf{ST}   & 306:30 & 318:48 & 332:29  & 149:52  &350:19   & 325:29& 286:39 & 307:22&581:43& 570:32&706:18 & 635:05\\ \cline{2-14}
%                                   & \textbf{TC}   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00  & 0:00   & 0:00  & 0:00 & 0:00  & 0:00  & 0:00  \\ \cline{2-14}
%                                   & \textbf{TT}   & 68:19  & 67:51  & 74:44   & 32:15   &80:51    & 76:13 & 35:54  & 35:28 &56:50 & 57:22 & 70:57 & 75:48 \\ \cline{2-14}
%                                   & \textbf{\#HF} &   -    & -      & -       & -       &   -     &  -    &   -    &   -   &  -   &   -   &   -   &   -   \\ \cline{2-14}
%                                   & \textbf{TF}   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00  & 0:00   & 0:00  & 0:00 & 0:00  & 0:00  & 0:00  \\ \cline{2-14} \hline 
% % ========================================================================================================================
%     \multicolumn{1}{l|}{}& \textbf{Alg.}
%     & \textbf{EX} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV}
%     & \textbf{EX} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV} \\ \hline
%     \multirow{13}{1cm}{\textbf{Open Chord}
%       % \newline \#S = 10K
%     \newline \#Agents = 2
%     \newline \#Rtry = N/A
%     \newline Qrm = N/A}           %                  EX1      DB1     DP1        TD1      IR1       LV1     EX2       DB2     DP2     TD2     IR2      LV2
%                                   & \textbf{\#S}  & 18,396 & 18,396 &  5,926  & 2,633   &  1,935  & 21    & 50K    &  50K  &  50K   &  50K  & 50K   & 71    \\ \cline{2-14}
%                                   & \textbf{\#IH} &   0    &   0    &   0     & 0       &  0      &  0    & 0      & 0     & 0      &  0    &  0    &  0    \\ \cline{2-14}
%                                   & \textbf{\#UH} &  165   &  165   &   143   &  117    &  121    & 17    & 325    & 3557  & 1073   &  1034 & 1498  &  49   \\ \cline{2-14}
%                                   & \textbf{\#NL} &  17    &  17    &   16    &  14     &  12     &  4    &  15    &  357  &  181   &  163  & 295   &  1    \\ \cline{2-14}
%                                   & \textbf{NL/UH}&  10.3\%& 10.3\% & 11.19\% & 11.97\% &  9.92\% &23.53\%& 4.62\% &10.04\%&16.87\% &15.76\%&19.69\%& 2.04\%\\ \cline{2-14}
%                                   & \textbf{UH/S} &  0.9\% & 0.9\%  &  2.41\% & 4.44\%  &  6.25\% &80.95\%& 0.65\% & 7.11\%& 2.15\% &2.07\% & 3.0\% &69.01\%\\ \cline{2-14}
%                                   & \textbf{NL/S} & 0.09\% & 0.09\% &  0.27\% & 0.53\%  &  0.62\% &19.05\%& 0.03\% & 0.71\%& 0.36\% & 0.33\%& 0.59\%& 1.41\%\\ \cline{2-14}
%                                   & \textbf{TS}   & 5:30   & 5:34   & 0:43    & 0:10    & 0:06    & 0:00  & 73:29  & 34:01 & 50:48  & 60:03 & 100:43& 0:00  \\ \cline{2-14}
%                                   & \textbf{ST}   & 18:25  & 17:56  & 2:04    & 0:34    & 0:24    & 0:00  & 323:39 & 138:25& 194:59 & 214:55& 359:59& 0:00  \\ \cline{2-14}
%                                   & \textbf{TC}   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00  & 0:00   & 0:00  & 0:00   & 0:00  & 0:00  & 0:00  \\ \cline{2-14}
%                                   & \textbf{TT}   & 5:30   & 5:34   & 0:43    & 0:10    & 0:06    & 0:00  & 73:29  & 34:02 & 50:48  & 60:03 & 100:43& 0:00  \\ \cline{2-14}
%                                   & \textbf{\#HF} &   15   &   15   &  12     &    10   &  12     &   0   & 15     &   1   &  2     &  9    &   1   &   22  \\ \cline{2-14}
%                                   & \textbf{TF}   & 0:00   & 0:00   & 0:00    & 0:00    & 0:00    & 0:00  & 0:00   & 0:00  & 0:00   & 0:00  & 0:00  & 0:00  \\ \cline{2-14} \hline
% % ========================================================================================================================
%     \multicolumn{1}{l|}{}& \textbf{Alg.}
%     & \textbf{EX} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV}
%     & \textbf{EX} & \textbf{DB} & \textbf{DP} & \textbf{TD} & \textbf{IR} & \textbf{LV} \\ \cline{2-14}

%   \end{tabular}
%   \caption{\scriptsize
%     This table shows 7 schedulers bench marked against 5
% distributed systems. The following is the legend for the symbols in the table:
% \textbf{Schedulers:} (EX) Exhaustive, (DB)
% Delay-Bounded, (DP) DPOR, (TD) TransDPOR, (IR) IRed , (LV)
% LiViola. \textbf{Per Benchmark symbols/numbers:} (\#Inv.) No. of
% Invocations, (R-W) the comparison of reads requests compared to write
% requests, (\#S) No. of Schedules, (\#UH) No. of Unique Histories,
% (\#NL) No. of Non-Linearizable histories, (NL/UH) None-Linearizable to
% Unique Histories, (\#IH) No. of Incomplete histories, (NL/S) ration of
% Non-Linearizable histories to No. of Schedules, (UH/S) Ration of
% No. of Unique Histories to No. of Schedules generated, (\#Rtry) No. of
% Retries, (Qrm) number of agents forming the Quorum if applicable, (TS)
% Time to generate all Schedules (mm:ss), (ST) time to produce same
% schedules by an otherwise a stateless variant of the algorithm, (TC)
% Time to check all unique histories (mm:ss), (TT) Total Time = TS + TC
% (mm:ss),(\#HF) No. of histories until first buggy history,(TF) time to
% find the First buggy history by WGL algorithm (mm:ss), that is the sum
% of time needed to check all histories before and including the first
% buggy one. Note that the number of agents in all these benchmarks was
% limited to 5. The subcolumns headers e.g. 2r+1w stands for 2 reads and
% 1 write test harness.
%   } % end caption
%   \label{big:table:benchmarks}
% \end{table}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:

==> tables/table-args.tex <==
\begin{table*}[ht]
  \centering
  \begin{tabular}{| c || l |}
    \hline
    \textbf{Argument} & \textbf{Description} \\
    \hline
    \hline
     \textbf{boot-sequence=spec} & its format not needed
                              to be discussed here. We will add it later.\\
    \hline
    \textbf{explore-boot=Y/N}  & need scheduler explore the boot sequence for violations or not.\\
    \hline
    \textbf{ds-type=ds-name}  & data structure this distributed system
                                represents e.g. queue, set, kv,
                                \ldots, etc.\\
    \hline
    \textbf{check=name} & scheduler name e.g. \texttt{linearizability}.\\
    \hline
    \textbf{dropping=N}  & \shortstack[l]{number of dropped messages per
                           communication round (e.g. a repeated \\request followed by one or more
    replies)}\\
    \hline
    \textbf{retries=N}& goes hand in hand with \texttt{dropping}.\\
    \hline
    \textbf{duplicates=Y/N} & deduplication on server
                              sides checking enabled. \\
    \hline
    \textbf{cduplicates=Y/N} & deduplication on client
                               sides checking enabled. \\
    \hline
         \textbf{quorum=p} & \shortstack[l]{what percentage of the
                             nodes bigger than 'p' forms a quorum,
                             it auto-enables \\ quorum-based exploration. \texttt{p} ranges between
    0 to 1.}\\
    \hline
     \textbf{include=Expr/List} & \shortstack[l]{an expression over node-identifiers
                                  (actor/agent names) that should be \\ considered as nodes belonging to
    this distributed store. Can be an explicit \\list of names/ids.}\\
    \hline
    \textbf{exclude=Expr/List}  & similar to \texttt{include} but for
                                  exclusion of nodes. \\
    \hline
    \textbf{reordering=p2p/np2p}  & \shortstack[l]{reordering of message delivery
    needs be explored or not, point-to-point \\order or no-point-to-point
    order needs be considered.} \\
    \hline
    \textbf{api-modify} & \shortstack[l]{operations on the distributed store which
  is specified as a list of list of \\ strings. Each inner list is of the
  format: \texttt{op-name, arg1, arg2, \ldots, argn}} \\
    \hline
\textbf{api-read}  & \shortstack[l]{same as \texttt{api-modify}. Both read and
  modify request have to be followed \\with an acknoledgment.} \\
    \hline
  \end{tabular}
  \caption{Arguments and their descriptions}
  \label{tab:args}
\end{table*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> tables/table-interference.tex <==
\begin{table}[htb!]
  \centering
  \footnotesize
  \begin{tabular}{c || c | c | c | c | c | c | c | c | c | c | c | c | c }
    
    & \rotatebox{90}{boot-seq}%     % 1
    & \rotatebox{90}{ds-type}%      % 2
    & \rotatebox{90}{check}%        % 3
    & \rotatebox{90}{dropping}%     % 4
    & \rotatebox{90}{retries}%      % 5
    & \rotatebox{90}{duplicates}%   % 6
    & \rotatebox{90}{cduplicates}%  % 7
    & \rotatebox{90}{quorum}%       % 8
    & \rotatebox{90}{include}%      % 9
    & \rotatebox{90}{exclude}%      % 10
    & \rotatebox{90}{reordering}%   % 11
    & \rotatebox{90}{api-modify}%   % 12
    & \rotatebox{90}{api-read} \\  % 13
    \hline
    \hline 
    Subject
    & 2,4
    & 1,2
    & 1,2
    & 1,2
    & 1,2
    & 1,2
    & 1,2
    & 1,2
    & 1,4
    & 1,4
    & 1,2
    & 1,2
    & 1,2\\
    \hline
    Client
    & % no dependency
    & 1,3
    & % no dependency
    & \makecell{1,2,\\4}
    & \makecell{1,2,\\3,4}
    & \makecell{1,2,\\3,4}
    & \makecell{2,3,\\4}
    & \makecell{1,2,\\3,4}
    & % no dependency
    & % no dependency
    & \makecell{1,2,\\4}
    & 1,3
    & 1,3\\
    \hline 
    Scheduler
    & \makecell{1,2,\\4}
    & \makecell{1,2,\\3,4}
    & 2,3 % means we need a scheduler per datastructure, then combine them
    & \makecell{1,2,\\4,5}
    & \makecell{1,2,\\4,5}
    & \makecell{1,2,\\4,5}
    & \makecell{1,2,\\4,5}
    & \makecell{1,2,\\4,5}
    & 2,4
    & 2,4
    & \makecell{1,2,\\4,5}
    & \makecell{2,4,\\5}
    & \makecell{2,4,\\5}\\
  \end{tabular}
  \caption{Arguments vs. affected behavior and/or implementation of
    subject, scheduler, and clients, given one scheduler
    implementation per data structure type under check. The legend of
    the symbols is read column-to-row direction and is as follows:  
    1. Depends on the static-time behavior/implementation of the subject
    2. Affects the runtime behavior/state-evolution
    3. Affects the static-time behavior/implementation
    4. Affects which agents are explored, given current global state
    5. Depends on client implementation.}
  \label{tab:interference}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../liviola"
%%% End:


==> tool.tex <==


% ----------------------------------------
\subsection{Complexity of Assumptions Combinations}
\label{sec:assumptions}
% ----------------------------------------
Before we start detailing the tool, lets take a look at the complexity
level we are dealing with to appreciate the value of automating the
process.
%
In order to cut on the numerous variables, which usually depends on
implementation trade offs decided by developers, we provide
\emph{three sets} of arguments to be provided to the front-end.
%
In turn, these arguments specify what specific most-generic client to
be used, what agents/processes to target as a subject data store, and
how the scheduler will boot them so that it explores the state space
in a smarter manner.
%
Some arguments affect more than one aspect of the tool, this is
summarized in Table~\ref{tab:interference}.%  while a description of all
% possible arguments can be found in Table~\ref{tab:args}

Based on Table~\ref{tab:interference}, the combinatorial complexity of
assumptions and options is huge. An estimate of the variation of
clients (a scheduler) implementations follows:
\begin{displaymath}
    \shortstack[l]{
      $|behaviors-explored| = |retries| \times |timed-actions|$ \\
      $|boot-variations| \times |droppings| \times |duplicates|$ \\
      $\times |quorum-combinations| \times |Agents| \times |reordering|$\\
      $ \times |invocations|\times |Internal-messaging|$\\
      $\times |Partitions|$}
\end{displaymath}
Then, based on those behaviors, how many combinations of scheduler
behaviors are there? Regardless of the fact that we fixed clients
implementations (a), and assumptions (d) in Fig~\ref{fig:args} and
omitted developer client-implementation (c), there is still enormous
state space to explore.
\input{tables/table-interference}
%
In order to manage the complexity modularily, Fig~\ref{fig:args} shows
how each of the set-of-assumptions/arguments affects the behavior
(implementation) of schedulers, clients and the extraction of subject
nodes in the target system.
%
Systems arguments (c), such as \texttt{include} and \texttt{exclude},
limits the exploration of the schedule to certain nodes (the target
agents that represent the ADT implementation).
%
Assumptions (d), change the behavior of scheduler exploration
algorithm and of clients.
%
An example of such assumptions are \texttt{duplication} handling and
\texttt{dropping}.
%
Clients (a) interact with the subject distributed system as the
scheduler (b) sees fit based on the assumptions and the scheduler
arguments.
%
Hence, clients are synthetic and their implementation is left
completely out in favor of the scheduler behavior.
%
That is, the scheduler acts on behalf of these clients, but maintains
a bench of agents to interact (i.e. send and receive invocations and
responses, respectively).
%
The rest is handled by the scheduler/algorithm.
%
Examples of scheduler arguments include \texttt{api-modify},
\texttt{api-read}, \texttt{quorum}.
%
That is, what message identifiers (regex) is considered an
invocation, and which ones are responses. Also, how do the harness
map to those clients are all specified in a harness file with a
specific format.

Table~\ref{tab:interference} shows the dependencies between scheduler,
clients, subjects on one hand and the different assumptions on the
other hand.
%
The manner these assumptions affect them, however, is not discussed
because it depends on the problem at hand.
%
For example in Linearizability checking, all the scheduler needs to
do is to check the client's queues, and picks the responses to add
response entries to the history.
%
Invocations are sent by these clients and are added at that time to
the history by the scheduler.
%
All internal messaging for the target agents is non of the clients'
business, it is solely the business of the scheduler's exploration
algorithm.

% % ----------------------------------------
% \subsection{Overview}
% \label{sec:tool-overview}
% % ----------------------------------------
% Diagram and explain it.

% Another Diagram: the assumptions

% The assumptions inter-relation table in my writeup, and the
% combinatorial explosion (state the rough equation).

% What is implemented so far. Limitations: no
% duplication/retries/dropped messages explored, front end is limited to
% some styles of coding (Heath should fill this one) (future work).

% The boundaries of the clients and nodes constituting the distributed
% store is then very clear.
% %
% The expressions provided can, not only distinguish whether the
% receiver/sender of requests/responses is in the distributed store
% nodes, but also distinguishes client's events from these nodes' events.

% Remains to demarcate is what are the requests, what are the responses
% to these requests, and how to distinguish which response belongs to
% which request.
% %
% Requests are marked by each client (the message sender field), the
% destination node, and time associated with this event by the
% scheduler.
% %
% Reverse the source and destination of the communication, and replace
% the request with a response (and a later timestamp), and now we can
% determine which response is directed to which request.
% %
% Actually, in our harness we ask the user to provide the regular
% expression(s) that map response messages to what operation on the data
% structure.
% %
% This way there is no ambiguity and it is straightforward for matching
% responses.
% %
% In a broadcast communication pattern, this is also achievable in the
% same manner.
% %
% Any other communication that doesn't agree with the \emph{reversal} or
% the regular expression is of another nature of communication e.g. could be a
% replication request, a two commit initiation/response request, or any
% internal communication
% \ldots{} etc.
% %
% One or many requests can be associated with one or many responses
% (acknowledgments) based on the \emph{sender} and \emph{destination}
% fields of the communication pattern(s) used\footnote{We have two only,
%   an ask and an async send}.
% %
% Any response \emph{must be} at a time later than any request, and vice
% versa.
% %
% There can't be a response to any request that is earlier than the
% request itself, unless that request is initiated by a different client, a
% concurrent one, and hence is directed to that concurrent client.
% %
% Once this is done, what remains is to utilize \emph{problem specific
%   knowledge} in order to determine
% where a linearizability violation may have happened.
% %
% For example, if a response appears in a history before its request, it
% is naturally a violation.
% %
% If, however, more than one response is received to only one request,
% that is not a violation.
% %
% There could be one sided retries from the store-side.
% %
% In the benchmarks we tried, we don't have this situation so we are not
% handling it.
% %
% However it is easy to modify the scheduler to handle it.
% %
% If there are multiple requests with the same sender, and no response
% interleaving these requests, then any response(s) received later to any of
% them satisfy all of them.
% %
% Otherwise, if the response received isn't for any of them, then another sender
% must have initiated another concurrent request and there has to be one
% matching this response.
% %
% In other words, if there isn't a request that matches this response
% in any of the clients, then it is a linearizability violation.
% %
% More specific knowledge depends on \emph{what} the distributed store
% represents (a set, register, \ldots{} etc) and what was observed (or
% can be observed predictably by linearizability checker) that doesn't
% agree with the data structure the distributed system represents.
% %
% \section{The Tool: IRed}
% \label{sec:tool}

% \input{figures/tool-fig}
% \input{figures/args-fig}

% \textcolor{red}{Outline}
% \begin{itemize}
% \item The Tool workflow, diagram, and high level
%   description. In this, describe in subsections (detail) how each
%   step takes its input, transforms it, and passes it to the next
%   phase of the pipeline.
% \item Add a note mentioning how our framework simplifies the implementation of
%   each subsequent algorithm by reusing implementations of the ones
%   before it.
% \item Each alg. explores Smaller state-space and little to no loss of
%   precision (interesting schedules).
% \item the state of the art is TransDPOR. Reason is in the following
%   note (regarding all linearizability violation is an internal race made
%   observable to clients through the ADT API, not all internal races are
%   linearizability violations though). Does LiViola improve over it? how
%   if so (differences, and an example showing improvement)? and evidence
%   is shown in the evaluation section.
% \end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "liviola"
%%% End:

% LocalWords:  combinatorial


==> wgl-intuitively.tex <==
\subsection{WGL: Intuitively with Examples}
\textcolor{red}{Mo: Ryan says add what Pcomp means, complexity
  analysis in terms of history length, and that it is a decision
  procedure}

Lets walk through few examples to show how WGL~\cite{lowe:wgl:linearizability}
works, examples shown in Figure\ref{fig:algorithm:example}.

%
Note that the letter \texttt{p} in the figure  indicates a \emph{put}
operation on a map, and the letter \texttt{g} indicates a \emph{get}
operation on the map abstract data structure. 
%
Lets begin with the example history of Figure\ref{fig:wgl1}. The
history can textually be written (and this is how the algorithm gets it
as a list of events): put(k1,1), ok(), get(k1), get(k1), ok(1), ok(1).
%
Each horizontal line corresponds to a process, different horizontal lines
correspond to different processes.
%
Time flows from left to right, and operations from different processes
can overlap, but operations from the same process can never overlap.
%
That is, each process can invoke one operation and unless its
completion was satisfied (i.e. response), it can not invoke another
operation.
%
In order to do so, another process needs to invoke the concurrent
operation.
%


%
\textbf{WGL Example1.}
So, going through history H1 (shown in Figure\ref{fig:wgl1}), WGL
algorithm picks the \emph{inv1} finds the matching response
(\emph{res1}) and performs the operation on the sequential map
implementation (called executable sequential specification) and checks
the response of the specification vs \emph{res1} (the concurrent
history response).
%
If the above, sequential vs concurrent histories agree, then that
specific invocation and response (call it operation) is linearizable,
so the WGL algorithm \emph{lifts}\footnote{lifting means removing the
  entry and its match, pushing it at top of a stack along with the
  state of the sequential specification was at before applying this
  operation. This is used for backtracking in case a response is
  encountered by the algorithm or the operation is not
  linearizable. So that, in turn, another re-arrangement of the
  entries is attempted by the algorithm.} it from the history H1 (i.e. removes
it) shortening the history and leaving only the operations that still need
to be checked for linearizability.
%
Luckily, H1 is linearizable, so WGL picks the first invocation that
happens to be \emph{inv2} and does the same with it as it did to
\emph{inv1}.
%
Remains \emph{inv3} and it does the same to it as it did to
\emph{inv1} and \emph{inv2}.
%
Since there is no more operations/entries in the history remaining,
the algorithm deems that history as \emph{linearizable}.
%
That took \emph{three} iterations from the WGL algorithm to linearize.

%
\textbf{WGL Example2.}
Now lets go through a bit longer example.
%
By now, the reader should know how WGL would go about the linearizable
history shown in Figure\ref{fig:wgl2}.
%
It would pick the first entry, happens to be \emph{inv1}, and finds
its match \emph{res1}, executes the specification, checks \emph{res1}
versus the specification response for the operation
(\emph{inv1}/\emph{res1}), if linearizable then lifts it, and so on.
%
It will require WGL \emph{six} iterations (with zero backtracking) to find it
is linearizable.
%

%
\textbf{WGL Example3.}
This is a longer example that is \emph{not} linearizable.
%
This would follow the algorithm shown in Figure\ref{alg:wgl:pcomp}.
%
This example is left as an exercise for the reader as we ran it
through our implementation of WGL and it checked the history shown in
Figure\ref{fig:wgl3} in \emph{fifteen} iterations.
%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "liviola"
%%% End:

